An action of the Witt algebra on Khovanov-Rozansky homology

We construct an action of the positive part of the Witt algebra on Khovanov--Rozansky $\mathfrak{gl}_N$-link homology and show that link cobordisms induce equivariant maps between twists of the homology. Moreover, the state spaces of simple webs are identified with standard representations of the Witt algebra on polynomials. Some simple relations to Lee homology and genus bounds are derived from the analysis of this presentation.

==> sch/def_dots_black_blank.tex <==
\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A);
  % \filldraw[draw= black, fill = black] (A) circle (.7mm)
  % node[below, yshift=-0.5mm] {$\omega$};
  \node (B) at (.55,.3) {$\deco_k P_{n-k}$};
\end{scope}


==> sch/def_dots_circle_black.tex <==
\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A);
  \filldraw[draw= black, fill = black] (A) circle (.7mm)
  node[below, yshift=-0.5mm] {$\omega$};
\end{scope}

==> sch/def_dots_circle_black_k.tex <==
\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A);
  \filldraw[draw= black, fill = black] (A) circle (.7mm)
  node[below, yshift=-0.5mm] {$\omega$};
  \node (B) at (.55,.3) {$\deco_k P_{n-k}$};
\end{scope}

==> sch/def_dots_circle_hollow_k.tex <==

\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A);
  \filldraw[draw= \crd, fill = white] (A) circle (.7mm)
  node[below, yshift=-0.5mm] {$\omega$};
  \node (B) at (.55,.3) {$\deco_k \deco_{n-k}$};
\end{scope}

==> sch/def_dots_circle_solid_k.tex <==
\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A);
  \filldraw[draw= \crd, fill = \csrd] (A) circle (.7mm)
  node[below, yshift=-0.5mm] {$\omega$};
  \node (B) at (.55,.3) {$\deco_k \hat{\deco}_{n-k}$};
\end{scope}

==> sch/def_dots_trian_hollow_n.tex <==
\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A); 
  \node (C) at (0.5,0.7) [draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=1.5pt]{};
  \node (D) at (0.5,0.7) [below,yshift=-0.5mm]{$\omega$}; 
  \node (B) at (.55,.3) {$\deco_n$};
\end{scope}

==> sch/def_dots_trian_solid.tex <==
\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A); 
  \node (C) at (0.5,0.7) [draw=\crd, fill=\csrd,regular polygon, regular polygon sides=3,inner sep=1.5pt]{};
  \node (D) at (0.5,0.7) [below,  yshift=-0.5mm]{$\lambda$};   
\end{scope}

==> sch/def_dots_trian_solid_n.tex <==
\begin{scope}
  \draw[thin] (0,0) rectangle (1,0.7);
  \draw[thick] (0,0.7) -- (1,0.7)  coordinate [pos=0.5] (A); 
  \node (C) at (0.5,0.7) [draw=\crd, fill=\csrd,regular polygon, regular polygon sides=3,inner sep=1.5pt]{};
  \node (D) at (0.5,0.7) [below]{$\lambda$};   
  \node (B) at (.55,.3) {$\hat{\deco}_n$};
\end{scope}

==> sch/foam_cup_deco_n+j.tex <==
\begin{scope}[font=\tiny]
  \draw (0,0) arc (180 :0: 0.5cm and 0.2cm) node[pos=0.3, draw=\crd, fill= \csrd, circle , inner sep=1.5pt]{} node[pos=0.3,below,yshift=1mm,xshift=2mm]{$-\frac{1}{2}$};
  \draw (0,0) arc (180 :0: 0.5cm and -0.6cm);
  \draw (0,0) arc (180 :0: 0.5cm and -0.2cm) node[pos=0.5, below,yshift=-.5mm] {$\deco_{n+i} $};
\end{scope}

==> sch/foam_cup_decorated.tex <==
\begin{scope}[font=\tiny]
  \draw (0,0) arc (180 :0: 0.5cm and 0.2cm) node[pos=0.3, draw=\crd, fill= \csrd, circle , inner sep=1.5pt]{} node[pos=0.3,below,yshift=1mm,xshift=2mm]{$-\frac{1}{2}$};
  \draw (0,0) arc (180 :0: 0.5cm and -0.6cm);
  \draw (0,0) arc (180 :0: 0.5cm and -0.2cm) node[pos=0.5, below,yshift=-.5mm] {$\deco_i $};
\end{scope}


==> sch/foam_cup_decorated_kl.tex <==
\begin{scope}
  \draw (0,0) arc (180 :0: 0.5cm and 0.2cm) node[pos=0.3, draw=\crd, fill= \csrd, circle , inner sep=1.5pt]{} node[pos=0.3,below,yshift=1mm,xshift=2mm]{$-\frac{1}{2}$};
  \draw (0,0) arc (180 :0: 0.5cm and -0.6cm);
  \draw (0,0) arc (180 :0: 0.5cm and -0.2cm) node[pos=0.5, below] {$\deco_{k+i} \antideco_l$};
\end{scope}


==> sch/foam_sing_saddle_empty.tex <==
\begin{scope}[yscale=0.5, xscale=0.5, font=\tiny]
  \begin{scope}
    \coordinate (At) at (0,0);
    \coordinate (Bt) at (0.5,1);
    \coordinate (Ct) at (3,1);
    \coordinate (Dt) at (2.5,0);
    \coordinate (Et) at (2,0.1);
    \coordinate (Ft) at (1,0.9);
  \end{scope}
  \coordinate (O) at (1.5, -0.5);
  \begin{scope}[yshift= -2cm]
    \coordinate (Ab) at (0,0);
    \coordinate (Bb) at (0.5,1);
    \coordinate (Cb) at (3,1);
    \coordinate (Db) at (2.5,0);
    \coordinate (Eb) at (0.8,0.5);
    \coordinate (Fb) at (2.2,0.5);
  \end{scope}

  \draw (Bt) -- (Bb) -- (Eb) -- (Fb) node[pos=0.5, below] {$a+b+c$}-- (Cb) -- (Ct) -- (Ft) -- (O);
  \filldraw[draw =  black, fill = white, fill opacity=0.5] (At) --
  (Et) -- (Dt) -- (Db) -- (Fb) -- (O) -- (Eb) -- (Ab) -- (At);
  \draw (Bt) -- (Ft)-- (Et) node[pos=0.5, xshift =0.2cm] {$c$} -- (O);

  \begin{scope}
    \node[xshift = -0.15cm] at (Ab) {$b$};
    \node[xshift = -0.4cm] at (Bt) {$a+c$};
    \node[xshift = 0.15cm] at (Ct) {$a$};
    \node[xshift = 0.35cm] at (Db) {$b+c$};
    
  \end{scope}

\end{scope}

==> sch/forktwist_3b.tex <==
\begin{scope}[xshift = 2.5cm]
	\coordinate (bl) at (0,  -1.5);
	\coordinate (br) at ( 1,  -1.5);
	\coordinate (bm) at (   0.5,-0.8);
	\coordinate (tl) at (0,   0.5);
	\coordinate (tr) at ( 1,   0.5);
	\coordinate (tm) at (   0.5, -0.2);

	\draw[<-]  (bl) .. controls +( 0, 0.5) and +(0,0) .. (bm);
	\draw[<-]  (br) .. controls +( 0, 0.5) and +(0,0) .. (bm);
	\draw[->-]  (0.5,1) .. controls +( -0.5, 0) and +(0,0) ..  (tl) .. controls +( 0, -0.5) and +(0,0) .. (tm)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, left]{$\lambda$};
	\draw[->-]  (0.5,1) .. controls +(0.5,0) and +(0,0) .. (tr) .. controls +( 0, -0.5) and +(0,0) .. (tm)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, right]{$\mu$};
	\draw [double] (bm) -- (tm) node[pos=0, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=0, right]{$s$};
	\draw[double] (0.5,2) -- (0.5,1) node[pos=1, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=1, right]{$- \overline{s}$};
\end{scope}


==> sch/hopflink_2.tex <==
\begin{scope}[xshift = 2.5cm]
	\draw[-] (0.5, 0.5) arc (0:180:0.5) -- (-0.5,0.5) .. controls +(0,-0.5) and +(0, 0.5) .. (0.5, -0.5);
	\fill[white] (0, 0) circle (1mm);
	\draw[-] (-0.5, -0.5) .. controls +(0,0.5) and +(0, -0.5) .. (0.5, 0.5);

	\draw (-0.5, 2) arc (-180:0:-0.5)  -- (-1.5,-0.5) arc (-180:0:0.5)  ;
	\draw (0.5, 2) arc (180:0:0.5)  -- (1.5,-0.5) arc (0:-180:0.5)  ;

	\draw[-]  (0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, right]{$\mu$};
	\draw[-]  (-0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, left]{$\lambda$};
	\draw[-][double] (0,1.5) -- (0,1)
		node[pos=1, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=1,yshift=1mm, right]{$s$};
\end{scope}


==> sch/hopflink_3.tex <==
\begin{scope}[xshift = 2.5cm]
	\draw[-] (0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (-0.5, 0.5);
	\fill[white] (0,0) circle (2mm);
	\draw[-] (-0.5, -0.5) ..controls +(0,0.3) and +(0,-0.3) .. (0.5,0.5);

	\draw (-0.5, 0.5) arc (-180:0:-0.5)  -- (-1.5,-0.5) arc (-180:0:0.5)  ;
	\draw (0.5, 0.5) arc (180:0:0.5)  -- (1.5,-0.5) arc (0:-180:0.5)  ;
\end{scope}


==> sch/hopflink_4.tex <==
\begin{scope}[xshift = 2.5cm]
	\draw (-0.5, 2) arc (-180:0:-0.5)  -- (-1.5,0.5) arc (-180:0:0.5)  ;
	\draw (0.5, 2) arc (180:0:0.5)  -- (1.5,0.5) arc (0:-180:0.5)  ;

	\draw[-] (0.5, 0.5) arc (0:180:0.5) -- (-0.5,0.5);
	\draw[-] (0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, right]{$\mu$};
	\draw[-]  (-0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, left]{$\lambda$};
	\draw[-][double] (0,1.5) -- (0,1)
		node[pos=1, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=1, yshift=1mm,right]{$s+1$};
\end{scope}


==> sch/red_dot_circular_hollow.tex <==
\begin{scope}
    \node(A) at (0,0) [draw=\crd, fill= white, circle , inner sep=2pt]{};
\end{scope}

==> sch/red_dot_circular_solid.tex <==
\begin{scope}
    \node(A) at (0,0) [draw=\crd, fill= \csrd, circle , inner sep=2pt]{};
\end{scope}


==> sch/red_dot_triangle.tex <==
\begin{scope}
    \node(A) at (0,0) [draw=\crd, fill=white, regular polygon, regular polygon sides=3,inner sep=1.2pt] {};
\end{scope}


==> sch/theta_blank.tex <==
\begin{scope}[xshift = 2.5cm]
	\draw (0,0) circle (0.5);
	\draw[double] (0,0.5) -- (0,-0.5);
\end{scope}


==> sch/theta_kl.tex <==
\begin{scope}[xshift = 2.5cm]
	\draw (0,0) circle (0.5);
	\draw (0:0.5) node[draw=black, fill= black, circle , inner sep=1.5pt]{} node[right]{$p_k$};
	\draw (180:0.5) node[draw=black, fill= black, circle , inner sep=1.5pt]{} node[left]{$p_l$};
	\draw[double] (0,0.5) -- (0,-0.5);
\end{scope}


==> sch/theta_left_kl.tex <==
\begin{scope}[xshift = 2.5cm]
	\draw (0,0) circle (0.5);
	\draw (180:0.5) node[draw=black, fill= black, circle , inner sep=1.5pt]{} node[left]{$p_l\hat{p}_k$};
	\draw[double] (0,0.5) -- (0,-0.5);
\end{scope}


==> sch/theta_right_kl.tex <==
\begin{scope}[xshift = 2.5cm]
	\draw (0,0) circle (0.5);
	\draw (0:0.5) node[draw=black, fill= black, circle , inner sep=1.5pt]{} node[right]{$p_l\hat{p}_k$};
	\draw[double] (0,0.5) -- (0,-0.5);
\end{scope}


==> sch/toruslink_4.tex <==
\begin{scope}[xshift = 2.5cm]

	\draw[-] (0.5, 0.5) arc (0:180:0.5) -- (-0.5,0.5);

	\draw[-] (0.5,0.5) -- (0.5,-2.5);
	\draw[-] (-0.5,0.5) -- (-0.5,-2.5);

	\draw[-]  (0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, right]{$\mu$};
	\draw[-]  (-0.5, 2) .. controls +( 0, -0.5) and +(0,0) .. (0,1.5)
		node[pos= 0.35 , draw=\crd, fill=white,regular polygon, regular polygon sides=3,inner sep=0.9pt] {} node[pos=0.3, left]{$\lambda$};
	\draw[-][double] (0,1.5) -- (0,1)
		node[pos=1, draw=\crd, fill= white, circle , inner sep=1.5pt]{} node[pos=1,yshift=1mm, right]{$s+m-1$};

	\draw[->-] (-0.5, 2) arc (-180:0:-0.5)  -- (-1.5,-2.5) arc (-180:0:0.5)  ;
	\draw[->-] (0.5, 2) arc (180:0:0.5)  -- (1.5,-2.5) arc (0:-180:0.5)  ;
\end{scope}


==> sch/zero_cohomo.tex <==
\begin{scope}
  \coordinate (bl) at (-0.5, -1);
  \coordinate (br) at ( 0.5, -1);
  \coordinate (bm) at (  0,-0.3);
  \coordinate (tl) at (-0.5,  1);
  \coordinate (tr) at ( 0.5,  1);
  \coordinate (tm) at (  0, 0.3);
  \draw[>-]  (bl) .. controls +( 0, 0.5) and +(0,0) .. (bm);
  \draw[>-]  (br) .. controls +( 0, 0.5) and +(0,0) .. (bm);
  \draw[<-]  (tl) .. controls +( 0, -0.5) and +(0,0) .. (tm);
  \draw[<-]  (tr) .. controls +( 0, -0.5) and +(0,0) .. (tm);
  \draw [double] (bm) -- (tm);
\end{scope}
